4D-StOP: Panoptic Segmentation of 4D LiDAR using Spatio-temporal Object Proposal Generation and Aggregation

In this work, we present a new paradigm, called 4D-StOP, to tackle the task of 4D Panoptic LiDAR Segmentation. 4D-StOP first generates spatio-temporal proposals using voting-based center predictions, where each point in the 4D volume votes for a corresponding center. These tracklet proposals are further aggregated using learned geometric features. The tracklet aggregation method effectively generates a video-level 4D scene representation over the entire space-time volume. This is in contrast to existing end-to-end trainable state-of-the-art approaches which use spatio-temporal embeddings that are represented by Gaussian probability distributions. Our voting-based tracklet generation method followed by geometric feature-based aggregation generates significantly improved panoptic LiDAR segmentation quality when compared to modeling the entire 4D volume using Gaussian probability distributions. 4D-StOP achieves a new state-of-the-art when applied to the SemanticKITTI test dataset with a score of 63.9 LSTQ, which is a large (+7%) improvement compared to current best-performing end-to-end trainable methods. The code and pre-trained models are available at: https://github.com/LarsKreuzberg/4D-StOP.

==> tables/per_category_class_test.tex <==
%##########################################################################################

\begin{table}[ht!]
\renewcommand{\arraystretch}{1.2}
\center
\footnotesize{
\tabcolsep=0.40cm
\begin{tabular}{l c |c c} 
 \toprule
 {Category} & {\# Scans} &  $\mathrm{S_{assoc}}$ & $\mathrm{S_{cls}}$ \\
 \midrule
 \multirow{2}{*}{Car} & {2} & {0.78} & {0.97} \\
 {} & {4} & {0.79} & {0.97} \\ \hline
 \multirow{2}{*}{Truck} & {2} & {0.48} & {0.53} \\
 {} & {4} & {0.56} & {0.46} \\ \hline
 \multirow{2}{*}{Bicycle} & {2} & {0.16} & {0.44} \\
 {} & {4} & {0.20} & {0.47} \\ \hline
 \multirow{2}{*}{Motorcycle} & {2} & {0.35} & {0.52} \\
 {} & {4} & {0.42} & {0.57} \\ \hline
 \multirow{2}{*}{Other-vehicle} & {2} & {0.35} & {0.55} \\
 {} & {4} & {0.42} & {0.53} \\ \hline
 \multirow{2}{*}{Person} & {2} & {0.34} & {0.57} \\
 {} & {4} & {0.40} & {0.55} \\ \hline
 \multirow{2}{*}{Bicyclist} & {2} & {0.62} & {0.59} \\
 {} & {4} & {0.66} & {0.62} \\ \hline
 \multirow{2}{*}{Motorcyclist} & {2} & {0.51} & {0.09} \\
 {} & {4} & {0.45} & {0.14} \\ \hline
 \multirow{2}{*}{Road} & {2} & {0.00} & {0.89} \\
 {} & {4} & {0.00} & {0.88} \\ \hline
 \multirow{2}{*}{Sidewalk} & {2} & {0.00} & {0.73} \\
 {} & {4} & {0.00} & {0.72} \\ \hline
 \multirow{2}{*}{Parking} & {2} & {0.00} & {0.66} \\
 {} & {4} & {0.00} & {0.66} \\ \hline
 \multirow{2}{*}{Other-ground} & {2} & {0.00} & {0.31} \\
 {} & {4} & {0.00} & {0.28} \\ \hline
 \multirow{2}{*}{Building} & {2} & {0.00} & {0.92} \\
 {} & {4} & {0.00} & {0.92} \\ \hline
 \multirow{2}{*}{Vegetation} & {2} & {0.00} & {0.84} \\
 {} & {4} & {0.00} & {0.84} \\ \hline
 \multirow{2}{*}{Trunk} & {2} & {0.00} & {0.69} \\
 {} & {4} & {0.00} & {0.69} \\ \hline
 \multirow{2}{*}{Terrain} & {2} & {0.00} & {0.68} \\
 {} & {4} & {0.00} & {0.68} \\ \hline
 \multirow{2}{*}{Fence} & {2} & {0.00} & {0.66} \\
 {} & {4} & {0.00} & {0.68} \\ \hline
 \multirow{2}{*}{Pole} & {2} & {0.00} & {0.57} \\
 {} & {4} & {0.00} & {0.58} \\ \hline
 \multirow{2}{*}{Traffic-sign} & {2} & {0.00} & {0.55} \\
 {} & {4} & {0.00} & {0.54} \\
 \bottomrule
\end{tabular}
\caption{\small\textbf{Per-category scores on SemanticKITTI 4D Panoptic Segmentation test set.}}
\label{tab:per_category_test_set}
}
\end{table}

%##########################################################################################

==> tables/per_category_class_validation.tex <==
%##########################################################################################

\begin{table}[ht!]
\renewcommand{\arraystretch}{1.2}
\center
\footnotesize{
\tabcolsep=0.40cm
\begin{tabular}{l c |c c} 
 \toprule
 {Category} & {\# Scans} &  $\mathrm{S_{assoc}}$ & $\mathrm{S_{cls}}$ \\
 \midrule
 \multirow{2}{*}{Car} & {2} & {0.87} & {0.97} \\
 {} & {4} & {0.87} & {0.97} \\ \hline
 \multirow{2}{*}{Truck} & {2} & {0.10} & {0.32} \\
 {} & {4} & {0.17} & {0.31} \\ \hline
 \multirow{2}{*}{Bicycle} & {2} & {0.49} & {0.75} \\
 {} & {4} & {0.62} & {0.66} \\ \hline
 \multirow{2}{*}{Motorcycle} & {2} & {0.89} & {0.85} \\
 {} & {4} & {0.98} & {0.76} \\ \hline
 \multirow{2}{*}{Other-vehicle} & {2} & {0.47} & {0.66} \\
 {} & {4} & {0.56} & {0.63} \\ \hline
 \multirow{2}{*}{Person} & {2} & {0.39} & {0.70} \\
 {} & {4} & {0.47} & {0.66} \\ \hline
 \multirow{2}{*}{Bicyclist} & {2} & {0.80} & {0.89} \\
 {} & {4} & {0.75} & {0.88} \\ \hline
 \multirow{2}{*}{Motorcyclist} & {2} & {0.30} & {0.00} \\
 {} & {4} & {0.76} & {0.00} \\ \hline
 \multirow{2}{*}{Road} & {2} & {0.00} & {0.93} \\
 {} & {4} & {0.00} & {0.93} \\ \hline
 \multirow{2}{*}{Sidewalk} & {2} & {0.00} & {0.45} \\
 {} & {4} & {0.00} & {0.47} \\ \hline
 \multirow{2}{*}{Parking} & {2} & {0.00} & {0.80} \\
 {} & {4} & {0.00} & {0.80} \\ \hline
 \multirow{2}{*}{Other-ground} & {2} & {0.00} & {0.01} \\
 {} & {4} & {0.00} & {0.00} \\ \hline
 \multirow{2}{*}{Building} & {2} & {0.00} & {0.90} \\
 {} & {4} & {0.00} & {0.90} \\ \hline
 \multirow{2}{*}{Vegetation} & {2} & {0.00} & {0.61} \\
 {} & {4} & {0.00} & {0.60} \\ \hline
 \multirow{2}{*}{Trunk} & {2} & {0.00} & {0.88} \\
 {} & {4} & {0.00} & {0.88} \\ \hline
 \multirow{2}{*}{Terrain} & {2} & {0.00} & {0.69} \\
 {} & {4} & {0.00} & {0.68} \\ \hline
 \multirow{2}{*}{Fence} & {2} & {0.00} & {0.74} \\
 {} & {4} & {0.00} & {0.76} \\ \hline
 \multirow{2}{*}{Pole} & {2} & {0.00} & {0.64} \\
 {} & {4} & {0.00} & {0.64} \\ \hline
 \multirow{2}{*}{Traffic-sign} & {2} & {0.00} & {0.49} \\
 {} & {4} & {0.00} & {0.51} \\
 \bottomrule
\end{tabular}
\caption{\small\textbf{Per-category scores on SemanticKITTI 4D Panoptic Segmentation validation set.}}
\label{tab:per_category_validation_set}
}
\end{table}

%##########################################################################################

==> tables/per_category_results_with4D-PLS.tex <==
%##########################################################################################

\begin{table}[htp]
\renewcommand{\arraystretch}{1.2}
\center
\footnotesize{
\tabcolsep=0.40cm
\begin{tabular}{l c |c c | c c | c c} 
 \toprule
 {} & {} & \multicolumn{4}{c}{\abbrev} & \multicolumn{2}{c}{4D-PLS}\\
 {} & {} & \multicolumn{2}{c}{Test Set} & \multicolumn{2}{c}{Validation Set} & \multicolumn{2}{c}{Validation Set}\\
 {Category} & {\# Scans} &  $\mathrm{S_{assoc}}$ & $\mathrm{S_{cls}}$ & $\mathrm{S_{assoc}}$ & $\mathrm{S_{cls}}$ & $\mathrm{S_{assoc}}$ & $\mathrm{S_{cls}}$ \\
 \midrule
 \multirow{2}{*}{Car} & {2} & {0.78} & {0.97} & {0.87} & {0.97} & 0.72 & 0.96 \\
 {} & {4} & {0.79} & {0.97} & {0.87} & {0.97} & 0.77 & 0.96\\ \hline
 \multirow{2}{*}{Truck} & {2} & {0.48} & {0.53} & {0.10} & {0.32} & 0.15 & 0.38 \\
 {} & {4} & {0.56} & {0.46} & {0.17} & {0.31} & 0.20 & 0.39 \\ \hline
 \multirow{2}{*}{Bicycle} & {2} & {0.16} & {0.44} & {0.49} & {0.75} & 0.36 & 0.72 \\
 {} & {4} & {0.20} & {0.47} & {0.62} & {0.66} & 0.59 & 0.71 \\ \hline
 \multirow{2}{*}{Motorcycle} & {2} & {0.35} & {0.52} & {0.89} & {0.85} & 0.56 & 0.88\\
 {} & {4} & {0.42} & {0.57} & {0.98} & {0.76} & 0.81 & 0.74\\ \hline
 \multirow{2}{*}{Other-vehicle} & {2} & {0.35} & {0.55} & {0.47} & {0.66} & 0.17 & 0.56\\
 {} & {4} & {0.42} & {0.53} & {0.56} & {0.63} & 0.38 & 0.55\\ \hline
 \multirow{2}{*}{Person} & {2} & {0.34} & {0.57} & {0.39} & {0.70} & 0.31 & 0.65 \\
 {} & {4} & {0.40} & {0.55} & {0.47} & {0.66} & 0.35 & 0.63 \\ \hline
 \multirow{2}{*}{Bicyclist} & {2} & {0.62} & {0.59} & {0.80} & {0.89} & 0.63 & 0.89 \\ 
 {} & {4} & {0.66} & {0.62} & {0.75} & {0.88} & 0.69 & 0.91 \\ \hline
 \multirow{2}{*}{Motorcyclist} & {2} & {0.51} & {0.09} & {0.30} & {0.00} & 0.10 & 0.00\\
 {} & {4} & {0.45} & {0.14} & {0.76} & {0.00} & 0.16 & 0.00 \\ \hline
 \multirow{2}{*}{Road} & {2} & {0.00} & {0.89} & {0.00} & {0.93} & - & - \\
 {} & {4} & {0.00} & {0.88} & {0.00} & {0.93} & - & - \\ \hline
 \multirow{2}{*}{Sidewalk} & {2} & {0.00} & {0.73} & {0.00} & {0.45} & - & - \\
 {} & {4} & {0.00} & {0.72} & {0.00} & {0.47} & - & - \\ \hline
 \multirow{2}{*}{Parking} & {2} & {0.00} & {0.66} & {0.00} & {0.80} & - & - \\
 {} & {4} & {0.00} & {0.66} & {0.00} & {0.80} & - & - \\ \hline
 \multirow{2}{*}{Other-ground} & {2} & {0.00} & {0.31} & {0.00} & {0.01} & - & - \\
 {} & {4} & {0.00} & {0.28} & {0.00} & {0.00} & - & - \\ \hline
 \multirow{2}{*}{Building} & {2} & {0.00} & {0.92} & {0.00} & {0.90} & - & - \\
 {} & {4} & {0.00} & {0.92} & {0.00} & {0.90} & - & - \\ \hline
 \multirow{2}{*}{Vegetation} & {2} & {0.00} & {0.84} & {0.00} & {0.61} & - & - \\
 {} & {4} & {0.00} & {0.84} & {0.00} & {0.60} & - & - \\ \hline
 \multirow{2}{*}{Trunk} & {2} & {0.00} & {0.69} & {0.00} & {0.88} & - & - \\
 {} & {4} & {0.00} & {0.69} & {0.00} & {0.88} & - & - \\ \hline
 \multirow{2}{*}{Terrain} & {2} & {0.00} & {0.68} & {0.00} & {0.69} & - & - \\
 {} & {4} & {0.00} & {0.68} & {0.00} & {0.68} & - & - \\ \hline
 \multirow{2}{*}{Fence} & {2} & {0.00} & {0.66} & {0.00} & {0.74} & - & - \\
 {} & {4} & {0.00} & {0.68} & {0.00} & {0.76} & - & - \\ \hline
 \multirow{2}{*}{Pole} & {2} & {0.00} & {0.57} & {0.00} & {0.64} & - & - \\
 {} & {4} & {0.00} & {0.58} & {0.00} & {0.64} & - & -\\ \hline
 \multirow{2}{*}{Traffic-sign} & {2} & {0.00} & {0.55} & {0.00} & {0.49} & - & - \\
 {} & {4} & {0.00} & {0.54} & {0.00} & {0.51} & - & - \\
 \bottomrule
\end{tabular}
\caption{\small\textbf{Per-category results on the SemanticKITTI test and validation set.}}
\label{tab:per_category_with4dpls}
}
\end{table}

%##########################################################################################
